SoK: Pitfalls in Evaluating Black-Box Attacks

Numerous works study black-box attacks on image classifiers. However, these works make different assumptions on the adversary's knowledge and current literature lacks a cohesive organization centered around the threat model. To systematize knowledge in this area, we propose a taxonomy over the threat space spanning the axes of feedback granularity, the access of interactive queries, and the quality and quantity of the auxiliary data available to the attacker. Our new taxonomy provides three key insights. 1) Despite extensive literature, numerous under-explored threat spaces exist, which cannot be trivially solved by adapting techniques from well-explored settings. We demonstrate this by establishing a new state-of-the-art in the less-studied setting of access to top-k confidence scores by adapting techniques from well-explored settings of accessing the complete confidence vector, but show how it still falls short of the more restrictive setting that only obtains the prediction label, highlighting the need for more research. 2) Identification the threat model of different attacks uncovers stronger baselines that challenge prior state-of-the-art claims. We demonstrate this by enhancing an initially weaker baseline (under interactive query access) via surrogate models, effectively overturning claims in the respective paper. 3) Our taxonomy reveals interactions between attacker knowledge that connect well to related areas, such as model inversion and extraction attacks. We discuss how advances in other areas can enable potentially stronger black-box attacks. Finally, we emphasize the need for a more realistic assessment of attack success by factoring in local attack runtime. This approach reveals the potential for certain attacks to achieve notably higher success rates and the need to evaluate attacks in diverse and harder settings, highlighting the need for better selection criteria.

==> A4_prior_submission.tex <==
\section*{Reviews from Prior Submission}

\newcommand{\response}[1]{\begin{mdframed}[linecolor=blue!80!black]#1\end{mdframed}}

We submitted a previous version of this paper to IEEE S\&P 2023 (\#411), which was dropped in the ``early reject" phase based on two reviews. This paper is substantially changed from that one, with a more clear focus, new attack taxonomy, and extensive improvements to the paper and experiments.

\shortsection{Major Concerns}
The reviewers identified several weaknesses in the paper. 
\begin{itemize}
    \item They raise concerns over a lack of preciseness for definitions on the quantity of the auxiliary data, as well as the definition of `representative' auxiliary data. 
    \item They raised concerns over the independence and usefulness of the axes proposed in our taxonomy, along with the motivation behind our experiments. 
    \item They suggested focusing on identifying technical gaps and challenges identified by our taxonomy.
    \item They suggested not to stick to seemingly obvious experimental results.
    \item They commented on the secondary focus on malware detection, which they felt undermined the general focus of the paper.
\end{itemize}


\shortsection{Summary of Changes}

\begin{itemize}
    \item We made our definition of the quantity of (initially available) auxiliary data more precise by elaborating on what each category value means (details in the point to point response below). We also added finer and more concrete categorization on the quality of the auxiliary data to avoid ambiguity in the word `representative'. 
    \item We changed our taxonomy based on reviewers' comments and our own reconsideration to ensure it grounds for the practical applications. Axes in the new taxonomy are mostly independent, and we explicitly discuss cases where potential interactions among some axes are possible.
    \item We highlighted the technical challenges in the currently under-explored areas.
    \item We added multiple new experiments that revolve around evaluation of current black-box attacks, and the conclusions are not obvious and are not reported in prior literature.
    \item We also narrowed our scope to focus on the image domain.
    \item We pointed out new insights for future research directions and proper evaluations.
\end{itemize}


Additionally, we have attached \textit{unedited reviews} from the previous submission below, along with in-line comments (in box) about what we have done to address them.

\subsection*{Reviewer A}
Overall merit: 1. Reject,
Reviewer expertise: 3. Knowledgeable,
Reviewer confidence: 2. Medium

\shortsection{Paper summary}
\textit{The paper offers an attacker-model taxonomy for black-box attacks on ML classifiers, surveys and categorizes work according to the taxonomy, uses the categorization to identify "whitespaces" in the literature, and reasons about their importance while sometimes suggesting baseline attacks within these whitespaces.}

\shortsection{Strengths}
\textit{The logical structure of the research, as well as the attacker-capability axes in the suggested taxonomy, mostly make sense and can be informative. The paper surveys many works, addresses both image- and malware-classification tasks, and does not shy away from adequate empirical evaluations where needed. Through its methodology, the paper arrives at at least 2 potentially-interesting technical questions that were previously under-studied: how to utilize data/model access to improve query-based attacks, and how to adapt attacks to top-K classifiers. It goes forward to show that combination of known techniques can successfully address these challenges, but argues that this may be studied further}

\shortsection{Weaknesses}
\textit{Most conclusions are far too obvious, for example that results cannot be assumed to transfer from simple to harder settings,}
\response{
In the original submission, the main message was to show that attacks claiming state-of-the-art performance should be made after testing on diverse set of experiments, instead of just testing on an almost solved setting of performing untargeted attacks against normal models with a sufficient perturbation budget. We believe evaluations in the original submission still uncover interesting trends, such as how relative ordering of attacks (based on their success rate) can change drastically between different settings (\Cref{sec:harder_settings}). Only when attacks are evaluated across a diverse set of models and settings (low perturbation budget, targeted attacks, against robust target models) does it become clear which attacks are actually best-performing.

In the current submission, we believe the conclusions (the three key insights from our proposed taxonomy \autoref{sec:taxonomy_insights} and the takeaway messages on proper evaluation of different baselines in \autoref{sec:new_eval}) are not obvious and provides valuable guidance for the community. 
} 

\textit{or that there are important differences between domain-constrained settings (e.g. malware) and end-to-end-differentiable settings (images).}
\response{In our previous submission, we include experiments (along with categorization of attacks) for the malware domain as well, demonstrating how most techniques for black-box attacks under image-based attacks do not easily transfer to malware-based classifiers. We have since removed analyses around the malware domain, and instead focused solely on image-based classifiers.}

\textit{Large portions of the paper (IV.A, IV.B, spanning almost 4 pages) lengthily report experiments whose motivation is unclear and whose conclusions are the obvious ones above}
\response{We revised our paper to avoid having a centralized experiment section. Instead, in the current submission, we break down each relevant experiment so that, they immediately follow the main point we are making.

In the previous submission, the experiments on transfer attacks in Section IV.A was to argue that, attacks should be evaluated carefully under diverse settings to truly verify the attack effectiveness, 
This argument has now become the third message (takeaway in \Cref{sec:harder_settings}) in the current submission. The message in our current submission is also enriched with two other points that show, 1) running attacks based on runtime metric can unlock the potential of some attacks, and 2) we still do not have a good way to decide when to stop local attacks to generate the best candidate adversarial examples for transfer attacks. We believe these messages are not obvious.

Experiments related to Section IV.B in the previous submission are removed from our current submission. In the previous submission, we conducted experiments in the `limited' query-setting, which used to be one value in the axis of `type of interactive queries' to the target, but now has been removed from the taxonomy and now only contains `Interactive queries' and `No interactive queries'. In this experiment in limited query setting in the original submission, we compare the bayesian optimization attack (named as BayesOpt, which is intended for low-query setting) and the generally efficient Square Attack \cite{andriushchenko2020square} attack and aim to reemphasize the importance of comparing different attacks in diverse (untargeted and targeted) settings as depending on the settings, attack effectiveness can change significantly. Another motivation of this experiment was to check if the BayesOpt attack is truly better than the Square Attack, as the former did not compare to the latter at the submission (Square Attack appears before the BayesOpt attack). Again, this experiment no longer exists in the current submission.
}

\textit{The "limited-query" setting also takes up a central role in the paper, but makes no sense to me: first, the line between limited-query and unlimited-query access is arbitrarily drawn. Second, attacks that use query access report the required number of queries as a metric, and do investigate the trade-off between the minimal number of queries and attack success. So we already know what is possible given just limited queries, and I do not see why the limited-unlimited distinction is useful}
\response{Based on reviewer feedback and re-evaluation of the taxonomy, we switched from our previous 3 possibilities of \{no, limited, and unlimited query access\} to the target model, to interactive access (query-based attacks), and no interactive access (transfer attacks). For query-based attacks, we draw attention to the possibility of settings where adversaries have unlimited query access to target models in a black-box setting (e.g., model hosted in secure enclave), and adversaries under such settings would care more about time than iterations (\Cref{sec:runtime_query_exps}).}

\textit{Some experimental details are missing, for example used input transformations or gradient computations or how exactly attacks were chosen for experimentation (Sec IV.A)}
\response{We provide details on our experimental setup in \Cref{app:experiments}, including implementation details for attacks, models, and justifications for our choice of attacks in \Cref{sec:runtime_transfer_exps}.}

\textit{The missing logical piece in the paper’s structure is explicitly deriving technical gaps in research-community knowledge, from the identified gaps in literature coverage of the attacker models (along the paper’s own chosen taxonomy axes). Note the distinction between the two things -- some threat models may not be explored, but techniques can be trivially adapted to them. The paper does include some of this content (IV.C, see “strengths” above), but it is buried inside a catch-all “evaluation” section instead of being an integral, front-and-center part of the methodology, and inform the main conclusions}
\response{We dedicate an entire Section (\Cref{sec:taxonomy_insights} to discuss insights from the taxonomy in detail, explicitly talking about technical challenges in under-explored areas (and how trivial adaptations of existing attacks may be insufficient), while also discussing the possibility of combining attacks from different related fields like model extraction and model inversion. This also addresses the comments in the \textbf{Comments for Authors} below.}

\shortsection{Comments for author}
I encourage the authors to resubmit to Oakland next year, after addressing the above, especially the last weakness: what technical problems (e.g. utilizing top-K outputs to reduce queries, or utilizing data/model access to reduce queries) are under-addressed in the literature? Note that technical problems are different from gaps in threat-model exploration

minor/editorial:
p13 “rawy bytes"

\shortsection{Requested changes}
\textit{see weaknesses}

\subsection*{Reviewer B}
\textit{Overall merit: 1. Reject,  Reviewer expertise 2. Some familiarity,  Reviewer confidence: 2. Medium}

\shortsection{Paper summary}
\textit{The paper is an SoK on adversarial examples in the vision and malware domains. The taxonomy spans 4 axes, namely query access, API feedback, access to auxiliary data, and access to auxiliary models.}

\textit{I found the axis of the taxonomy of the paper to not be independent. For instance, auxiliary models may just as well provide auxiliary samples to the attack. Moreover, the specifications such as "limited samples" etc. are at best imprecise and often conflate assumptions about access to training data.}
\response{

We changed `auxiliary models' to `availability of pre-trained models' to ground the taxonomy closer to practical settings (where pretrained models, especially in the vision domain, are readily available) and explicitly distinguish between available models, and models that adversaries may train using auxiliary data. By setting the `availability of pretrained' models as a sub-axis, we ensure the 4 main axes in the current submission are as independent from each other as possible. However, the interaction among the quantity/quality of auxiliary data and the availability of pretrained models (see \Cref{sec:new direction}) might be unavoidable due to the nature of black-box attacks. We also changed possible values over the quantity of auxiliary data from 3 values of (none, limited, sufficient) to 2 (insufficient, sufficient), and elaborate on what the categories mean. The transition threshold between the two new values can be instantiated given a particular application setting (see details in \Cref{sec:quant aux data}).

}

\textit{Finally, the evaluation section was not nearly as comprehensive as I hoped it would be; given the title and the claims in the introduction. That is, I think, partially due to the way the taxonomy is set up, and partially due to the lack of focus of the paper. The paper is at the same time trying to create a useful taxonomy for adversarial examples in the traditional vision domain while running a parallel study on malware detection; and even introducing a new adversarial attack in Section 4.C. The result is that, unfortunately, I do not think the paper does any of the three in a polished way.}
\response{We shifted our focus to just the vision domain to allow more thorough analyses and evaluations. Our current experiments are well-motivated by gaps exposed by the proposed taxonomy, and revolve around the theme of current attacks sometimes using baselines from incorrect threat models, and how standardization of transfer attacks based on iterations is disconnected from what adversaries care about in maximizing attack success.}

\shortsection{Strengths}
\textit{The paper considers the application of attacks in more generalized settings and discusses their general merit. I think this is an important consideration in the era of hyper-specialized attacks.}

\shortsection{Weaknesses}
\textit{The paper lacks solid formulations for the terms of the trade it uses to describe the various attack. This is essential for a survey-style paper like this; as it is often taken to be a first point of entry to the field.}
\response{\Cref{sec:background} gives a necessary introduction to adversarial examples. \Cref{sec:method category} is dedicated to discussing attack method categories, across both transfer and query-based attacks. Additionally, \Cref{sec:evaluated attack background} contains brief descriptions of the attacks that we discuss and use in our experiments.}

\textit{"Transferability" is never really pinpointed in the context of adversarial examples
"sufficient" samples is not well-defined really. Neither is "representative." Especially for a unifying framework, it is important to be precise.
In defining an axis of evaluation, it is important to consider the interactions between these axes and how truly independent these axes are in a decision-making process}
\response{We include explicit definitions and discussions around adversarial examples in \Cref{sec:background}, for both targeted and untargeted settings. We also changed possible values over data quantity from 3 (none, limited, sufficient) to 2 (insufficient, sufficient), and elaborate on what each category means and how the transition threshold between two (values) can be concretely instantiated given a particular application setting (\Cref{sec:quant aux data}). The `Representative' auxiliary data in the original submission is also devided into three finder categories of `No', `Partial' and `Complete' overlap (in data features and/or label space) with the target training distribution. This way, we avoid the ambiguity of the single word `Representative' when describing the auxiliary data. 

Our current taxonomy was re-designed (from the prior taxonomy) to reflect practical settings better (e.g., setting the availability of pretrained models as a sub-axis to indicate that pretrained models can be abudantly available in image domain). It also takes special care of possible interactions between axes to make sure the main axes are as independent as possible each other. However, as discussed in  \Cref{sec:new direction}, the interaction between the quality/quantity of the auxiliary data (main axes) and the availability of pretrained models (sub-axis) might be unavoidable due to the nature of black-box attacks. 

}

\textit{The paper does not consider the effects that some choices for one axis can have on another}
\response{\Cref{sec:new direction} includes a detailed discussion on interactions among axes.}

\textit{The goal, and by extension, the audience of the taxonomy is not clear. By extension, it is never made clear why this particular taxonomy makes the most sense.}
\response{
We have revised our taxonomy based on reviewer's suggestions. The goal of the new taxonomy (in current submission) is to illustrate gaps in the threat space (from a practical point of view) while looking at attacks in the current literature and helping researchers be mindful of the threat space under which they propose and evaluate attacks, all while motivating research in areas that are currently unexplored and coincidentally the most interesting ones for practical adversaries.}

\textit{As a defender, targeted vs. untargeted is much more important in risk evaluation vs. access to auxiliary models}
\response{We included evaluations for targeted attacks, as well as attacks against adversarially robust models, and attacks under reduced (compared to the literature) perturbation budgets. The inclusion of such hard baselines is in fact now one of our key messages to researchers.}

\textit{- For instance, auxiliary models may just as well provide auxiliary samples to the attack
I do not think the "auxiliary data" axis is sufficiently explored}
\response{We revised our taxonomy to consider `Existence of Pretrained Models' as a sub-axis, and divided the original `Auxiliary Data' axis into two finer categories of `Quality' and `Quantity' of the auxiliary data, where the `Quality' of data initially available (i.e., the overlap between available auxiliary data, and the target model's training data (on a distribution level)) was missing from the previous submission.
We also include a detailed discussion centred around different possibilities of the
interaction between the pretrained (auxiliary) models and the quality and quantity of the auxiliary data in \Cref{sec:new direction} (e.g., pretrained models in providing auxiliary samples).} 

\textit{It does not address the different possible oracles
Besides the number of samples, the distinction between randomly sampled datasets is not made clear - An important missing access level on data is random-access oracle v.s. active learner}
\response{A noisy oracle that provides noisy labels corresponding to auxiliary data available with the adversary, is covered by the case where the quality of auxiliary data is ``low" in our new taxonomy (in current submission), since a noisy oracle would correspond to a mismatch in the label distribution. Regarding active-learning based oracles, we do include analyses that mention model-inversion and model-extraction attacks (whose attack process incorporates active learning principle) as related fields which can potentially interplay with black-box attacks.}

\textit{Important to consider the "quality" of the data (task defined; e.g. adversarial examples) vs. quantity}
\response{Our current taxonomy includes an axis each dedicated to the quality, and is independent from the quantity of auxiliary data.}

\textit{There is a "secondary" focus on malware detection in particular which undermines the general focus of the paper}
\response{We agreed with the reviewer's suggestion and removed malware-related experiments and discussions, and instead focused on the image domain.}

\textit{While the insights on the need for more work on "Top-K Predictions" is interesting (Section III.G.3); I think a highly relevant problem, that of "multi-label" top-k predictions is missing. Given that the traditional multi-class neural network predictions are only calibrated for the correct class; any well-calibrated model producing top-k predictions is likely to take advantage of multiple labels. There are works such as "TkML-AP: Adversarial Attacks to Top-k Multi-Label Learning" that authors are advised to include in their discussion.}
\response{The reference paper considers a setting different from ours, where each instance is now associated with multiple grountruth labels and the attacker aims to change all the (correct) \topk\ prediction labels by generating the perturbations and the attackers have \emph{white-box} access to the target model. In contrast, we consider \emph{black-box attacks} against a target model that only has one ground-truth labels. However, the techniques proposed in this paper might help attacks in \topk setting given sufficient enough adaptation and we added discussion in \Cref{sec:unexplored areas}.
}

\shortsection{Minor issues:}

\textit{"Whitebox" and "Blackbox" are used inconsistently: "The gradient estimation attacks submit queries to the target model to estimate the gradient of the target model and use the estimated gradient to perform white box attacks [23 ]" and "One exception uses black-box interpretability tools that estimate gradient-related statistics [128]"}
\response{Our intention was to talk about black-box gradient-estimation attacks; we have made the distinction explicit (wherever discussed) in the current version.}

\shortsection{Comments for author}

\textit{Consider quantifying "access to similar models" as having a (possibly noisy) oracle
There is a short mention of the oracle model in Section III.G.1 that I invite the authors to expand on: "If there are pre-trained models available, it is also feasible to take advantage of the limited available samples to generate high-value queries to the target model that reveal useful information, which is then related to model stealing attacks [114] and active learning [16]."}
\response{We changed `access to similar models' to a different sub-axis centred around availability of pretrained models, to differentiate such models from ones that adversaries may train using the available auxiliary data. Our current version indeed includes a detailed discussion on utilizing model stealing and model extraction attacks to potentially improve black-box attacks, and the state-of-the attacks in each field also incorporates the active learning principle. 
}

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

